Multi-domain semantic segmentation with pyramidal fusion

We present our submission to the semantic segmentation contest of the Robust Vision Challenge held at ECCV 2020. The contest requires submitting the same model to seven benchmarks from three different domains. Our approach is based on the SwiftNet architecture with pyramidal fusion. We address inconsistent taxonomies with a single-level 193-dimensional softmax output. We strive to train with large batches in order to stabilize optimization of a hard recognition problem, and to favour smooth evolution of batchnorm statistics. We achieve this by implementing a custom backward step through log-sum-prob loss, and by using small crops before freezing the population statistics. Our model ranks first on the RVC semantic segmentation challenge as well as on the WildDash 2 leaderboard. This suggests that pyramidal fusion is competitive not only for efficient inference with lightweight backbones, but also in large-scale setups for multi-domain application.

==> imports/figures.tex <==
%\usepackage{floatrow} 				% centriranje svih slika
\usepackage{float}					% figure [H]
\usepackage{graphicx} 				% includegraphics
%\usepackage{caption}			% subfigure
\usepackage{subcaption}			% subfigure
%\usepackage[export]{adjustbox} 	% http://ctan.org/pkg/adjustbox

\usepackage[section]{placeins}  % [section] for \FloatBarrier before every section 

\graphicspath{ {./figures/} }		% mapa sa slikama
%\let\oldincludegraphics\includegraphics
%\renewcommand{\includegraphics}[2][]{\oldincludegraphics[#1,max width=0.9\linewidth]{#2}}

%\usepackage{flafter} % floats after the first reference
    

==> imports/math.tex <==
% ULTIMATH


% redefinition of left and right to make spacing consistent
% https://tex.stackexchange.com/questions/2607/spacing-around-left-and-right/2610
\let\originalleft\left
\let\originalright\right
\renewcommand{\left}{\mathopen{}\mathclose\bgroup\originalleft}
\renewcommand{\right}{\aftergroup\egroup\originalright}

\usepackage{amsmath}
\usepackage{amssymb}  % loads amsfonts

% adding equation number inside align*
\newcommand\numberthis{\addtocounter{equation}{1}\tag{\theequation}}

\usepackage{mathtools}  % \coloneqq, smashoperator
%\usepackage{bm}
%\usepackage[utopia]{mathdesign}

%\usepackage{commath}  % calculus, perentheses
% https://tex.stackexchange.com/questions/135944/commath-and-ifinner/135985#135985
% instead of commath:
%% begin commath-fixed
\DeclareMathOperator{\dif}{d\!}
\DeclareMathOperator{\Dif}{D\!}

\makeatletter
\newcommand{\spx}[1]{%
	\if\relax\detokenize{#1}\relax
	\expandafter\@gobble
	\else
	\expandafter\@firstofone
	\fi
	{^{#1}}%
}
\makeatother

\newcommand\pd[3][]{\frac{\partial\spx{#1}#2}{\partial#3\spx{#1}}}
\newcommand\tpd[3][]{\tfrac{\partial\spx{#1}#2}{\partial#3\spx{#1}}}
\newcommand\dpd[3][]{\dfrac{\partial\spx{#1}#2}{\partial#3\spx{#1}}}

\newcommand{\md}[6]{\frac{\partial\spx{#2}#1}{\partial#3\spx{#4}\partial#5\spx{#6}}}
\newcommand{\tmd}[6]{\tfrac{\partial\spx{#2}#1}{\partial#3\spx{#4}\partial#5\spx{#6}}}
\newcommand{\dmd}[6]{\dfrac{\partial\spx{#2}#1}{\partial#3\spx{#4}\partial#5\spx{#6}}}

\newcommand{\od}[3][]{\frac{\dif\spx{#1}#2}{\dif#3\spx{#1}}}
\newcommand{\tod}[3][]{\tfrac{\dif\spx{#1}#2}{\dif#3\spx{#1}}}
\newcommand{\dod}[3][]{\dfrac{\dif\spx{#1}#2}{\dif#3\spx{#1}}}

\newcommand{\genericdel}[4]{%
	\ifcase#3\relax
	\ifx#1.\else#1\fi#4\ifx#2.\else#2\fi\or
	\bigl#1#4\bigr#2\or
	\Bigl#1#4\Bigr#2\or
	\biggl#1#4\biggr#2\or
	\Biggl#1#4\Biggr#2\else
	\left#1#4\right#2\fi
}
\newcommand{\del}[2][-1]{\genericdel(){#1}{#2}}
\newcommand{\cbr}[2][-1]{\genericdel\{\}{#1}{#2}}
\let\set\cbr
\let\event\cbr
\newcommand{\sbr}[2][-1]{\genericdel[]{#1}{#2}}
\newcommand{\intoo}[2][-1]{\mathinner{\genericdel(){#1}{#2}}}
\newcommand{\intcc}[2][-1]{\mathinner{\genericdel[]{#1}{#2}}}
\newcommand{\intoc}[2][-1]{\mathinner{\genericdel(]{#1}{#2}}}
\newcommand{\intco}[2][-1]{\mathinner{\genericdel[){#1}{#2}}}
\newcommand{\eval}[2][-1]{\genericdel.|{#1}{#2}}
\newcommand{\envert}[2][-1]{\genericdel||{#1}{#2}}
\let\abs\envert
\newcommand{\enVert}[2][-1]{\genericdel\|\|{#1}{#2}}
\let\norm\enVert
\newcommand{\fullfunction}[5]{%
	\begin{array}{@{}r@{}l@{}}
		#1 \colon #2 &{}\longrightarrow{}  #3 \\
		#4 &{}\longmapsto{} #5
	\end{array}
}
% parentheses from commath redefined to improve spacing because left and right were redefined, \midmid, new \tilde and \hat that don't make parentheses bigger
\newcommand{\ind}[1]{{\sbr{#1}}}
%% end commath-fixed

\usepackage{stmaryrd}  % \llbracket for \rrbracket, ...

%\newtheorem{definition}{Definicija}[section]
%\newtheorem{theorem}{Teorem}[section]
%\newtheorem{corollary}{Korolar}[theorem]

% More consistent fonts
\usepackage[OMLmathsfit]{isomath}  % \DeclareMathAlphabet ...
\usepackage{upgreek}

\DeclareMathAlphabet{\mathbbmsl}{U}{bbm}{m}{sl}
\DeclareMathAlphabet{\mathbbmb}{U}{bbm}{b}{it}
\DeclareMathAlphabet{\mathbbmssit}{U}{bbmss}{m}{it}

% common set?, distribution
\newcommand{\commset}[1]{\mathbbmb{#1}}
\newcommand{\distrib}[1]{\mathcal{#1}}

% sans-serif blackboard-bold
\newcommand{\mathsfbbit}[1]{\mathbbmssit{#1}}

% variable
\let\vec\relax
\let\set\relax
\newcommand{\vec}[1]{\boldsymbol{#1}}
\newcommand{\set}[1]{\mathbbmsl{#1}}

% constant
\newcommand{\const}[1]{\mathrm{#1}}
\newcommand{\cvec}[1]{\mathbf{#1}}
\newcommand{\cset}[1]{\mathbb{#1}}

% underlining (for random variables)
\newcommand{\nunder}[2][5]{\mathrlap{\mkern\the\numexpr#1/2mu\relax\underline{\phantom{\mathrm{#2}\mkern-#1mu}}}\mathrm{#2}}
\newcommand{\subline}[2][n]{%
    \makebox[\widthof{$#2$}/2]{}\mathclap{#2}%
    \text{\smash{\raisebox{0.04em}{% 0.04
        $\mathclap{\underline{\hphantom{#1}\vphantom{#2}}}$%
    }}}%
    \makebox[\widthof{$#2$}/2]{}%
}

% random variables (Dutch notation - J. Hemelrijk, underlining random variables)
% https://lingpipe-blog.com/2009/10/13/whats-wrong-with-probability-notation/
\newcommand{\rvarstyle}[1]{{{\subline[i]{#1}}}}
\newcommand{\rvar}[1]{\rvarstyle{#1}}
\newcommand{\rvec}[1]{\rvarstyle{\vec{#1}}}
\newcommand{\rset}[1]{\rvarstyle{\set{#1}}}
\newcommand{\var}[1]{{\color{red}#1}}

% linear algebra
\newcommand{\transpose}{\mathsf T}
\newcommand{\tp}{\transpose}

% calculus - commath: od, pd, md, dif
% parentheses - commath: del, cbr, sbr, envert, enVert

% named functions
\DeclareMathOperator{\softplus}{softplus}
\DeclareMathOperator{\softmax}{softmax}
\DeclareMathOperator{\logistic}{\sigma}
\DeclareMathOperator{\sgn}{sgn}
\DeclareMathOperator{\diag}{diag}
\DeclareMathOperator{\ReLU}{ReLU}
\DeclareMathOperator{\modfunc}{mod}

% operators
\DeclareMathOperator{\vecfunc}{vec}
\DeclareMathOperator*{\argmin}{arg\,min} % thin space
\DeclareMathOperator*{\argmax}{arg\,max}
\let\P\relax
\DeclareMathOperator{\P}{P}
\DeclareMathOperator{\p}{\mathrm{p}}
\DeclareMathOperator*{\E}{\mathrm{I\kern-.282em E}}
\DeclareMathOperator*{\D}{\mathrm{I\kern-.282em D}}
\DeclareMathOperator*{\Cov}{\mathrm{Cov}}
%\let\H\relax
\renewcommand{\H}{\mathrm{H}}
\newcommand{\h}{\mathrm{h}}
\newcommand{\I}{\mathrm{I}}
\newcommand{\Dist}{\mathrm{D}}  % D is for dispersion

% graphs
\newcommand{\pa}{\mathrm{pa}}
\newcommand{\ch}{\mathrm{ch}}
\newcommand{\pred}{\mathrm{pred}}
\renewcommand{\succ}{\mathrm{succ}}

% bracket operators
%\newcommand{\enangle}[1]{\mathinner{\left\langle{#1}\right\rangle}}
\newcommand{\enangle}[2][-1]{\genericdel\langle\rangle{#1}{#2}}
\newcommand{\enbbracket}[1]{{\mathinner{\left\llbracket{#1}\right\rrbracket}}}
\newcommand{\braket}[2]{\enangle{{#1}\middle|{#2}}}

%\let\mid\relax
%\newcommand{\mid}{\;|\;}  % spaces around not reduced in index
\newcommand{\midmid}{\;\middle|\;}

% hat and tilde
\let\oldhat\hat
\renewcommand{\hat}[1]{\vphantom{#1}\smash[t]{\oldhat{#1}}}
\let\oldtilde\tilde
\renewcommand{\tilde}[1]{\vphantom{#1}\smash[t]{\oldtilde{#1}}}
%\renewcommand{\tilde}[1]{\stackrel{\sim}{\smash{\mathcal{#1}}\rule{0pt}{1.1ex}}}
%\renewcommand{\tilde}[1]{\overset{\sim}{#1}}}
\let\oldwidetilde\widetilde
\renewcommand{\widetilde}[1]{\vphantom{#1}\smash[t]{\oldwidetilde{#1}}}

% special
%\newcommand{\funcdef}[3]{#1 \in (#2 \to #3)}
\newcommand{\funcdef}[3]{#1 \colon #2 \to #3}
\newcommand{\Dkl}[2]{\Dist_\mathrm{KL}\del{#1\;\middle\|\;#2}}
\newcommand{\C}{\cset{C}}
\newcommand{\R}{\cset{R}}
\newcommand{\Z}{\cset{Z}}
\newcommand{\N}{\cset{N}}
\newcommand{\dirac}{\updelta}

\newcommand\concat{\mathbin{+\mkern-10mu+}}

% machine learning evaluation
\newcommand{\TP}{\mathit{TP}}
\newcommand{\FP}{\mathit{FP}}
\newcommand{\TN}{\mathit{TN}}
\newcommand{\FN}{\mathit{FN}}
\newcommand{\FPR}{\mathit{FPR}}
\newcommand{\TPR}{\mathit{TPR}}
\newcommand{\AUROC}{\mathit{AUROC}}
\newcommand{\AUPR}{\mathit{AUPR}}
\newcommand{\AP}{\mathit{AP}}
\newcommand{\IoU}{\mathit{IoU}}
\newcommand{\mIoU}{\mathit{mIoU}}

% operators and relations
\newcommand{\bidot}{\mkern1.5mu{..}\mkern1.5mu}
%\newcommand\sheq{\mkern1.5mu{=}\mkern1.5mu}
%\renewcommand{\dots}{...}


% no vertical space stretching around display math
\usepackage[nodisplayskipstretch]{setspace}

\newenvironment{talign}
{\let\displaystyle\textstyle\align}
{\endalign}
\newenvironment{talign*}
{\let\displaystyle\textstyle\csname align*\endcsname}
{\endalign}


\usepackage{dashbox}%
%\newcommand\dashedbox[1][H]{\setlength{\fboxsep}{0pt}\setlength{\dashlength}{4pt}\setlength{\dashdash}{2pt} \dbox{\phantom{#1}}}
\newcommand\phbox[1][\phantom{:}]{\setlength{\fboxsep}{0.5pt}\setlength{\dashlength}{4pt}\setlength{\dashdash}{3pt} \raisebox{2pt}{\dbox{$\phantom{:}_{#1}$}}}
%\newcommand\dashedbox[1][H]{\setlength{\fboxsep}{0pt}\dbox{\phantom{#1}}}


==> imports/tables.tex <==
\usepackage{booktabs}  % from the template; table quality enhancement

\usepackage{multirow}
\usepackage{tabularx}
%\usepackage{tabu}
%\usepackage{makecell}

%\newcolumntype{P}[1]{>{\raggedright\let\newline\\\arraybackslash\hspace{0pt}}p{#1}}

%\renewcommand{\arraystretch}{1.1}
